Contextual Neural Model for Translating Bilingual Multi-Speaker Conversations

Recent works in neural machine translation have begun to explore document translation. However, translating online multi-speaker conversations is still an open problem. In this work, we propose the task of translating Bilingual Multi-Speaker Conversations, and explore neural architectures which exploit both source and target-side conversation histories for this task. To initiate an evaluation for this task, we introduce datasets extracted from Europarl v7 and OpenSubtitles2016. Our experiments on four language-pairs confirm the significance of leveraging conversation history, both in terms of BLEU and manual evaluation.

==> table-meanstats.tex <==
\setlength{\tabcolsep}{0.3pt}

\begin{table*}[t!]
\begin{minipage}{0.58\linewidth}
{\small
%\begin{table*}
%\begin{minipage}{0.55\linewidth}
%\centering
\begin{tabular}{c|c c c | c}
& \multicolumn{3}{c}{\textbf{Europarl}} & \multicolumn{1}{|c}{\textbf{Subtitles}}\\
\cline{2-5}
& \textbf{En-Fr} & \textbf{En-Et} & \textbf{En-De} & \textbf{En-Ru} \\
\hline
\hline
\multicolumn{5}{c}{\textbf{Train/Dev/Test}}\\
\hline
{\# Conversations} & {6997/140/209} & {4394/88/132} & 3582/70/108 & 23126/462/694 \\
%\# Sentences & 246540/4918/7818 & 174218/3158/5151\\
{\# Sentences} & {246k/4.9k/7.8k} & {174k/3.2k/5.2k} & 109k/2.1k/3.3k & 291.5k/5.9k/9k \\
%Joint Vocabulary Size & 29178 & 29240 & 29707\\
\hline
\hline
\multicolumn{5}{c}{\textbf{Train source-side}}\\
\hline
%\# Chapters & 6997 & 3582 & 4394\\
{\# Sentences (En/Fr)} & {139.8k/106.7k} & {130.6k/43.6k} & 55.5k/53.7k & 157.9k/133.6k \\
\hline
%\multicolumn{4}{c}{\textbf{Mean Statistics per Chapter}}\\
%\hline
%\# Sentences & 36.235 & 31.497 & 40.649\\
%\# English Sentences & 19.99 & 15.50 & 29.72\\
%\# Turns & 4.77 & 4.789 & 4.85\\
%\# English Turns & 2.706 & 2.356 & 3.44\\
%Turn Length & 7.119 & 6.160 & 7.918\\
%Turn Length (whole corpus) & 7.59 & 6.58 & 8.38\\
%\hline
\end{tabular}
}
\caption{General corpora statistics. \andre{these two tables are very cluttered. Format them differently? Maybe move some of these information to supplementary material?}}
\label{tab:data}
\end{minipage}
\hfill
\begin{minipage}{.33\linewidth}
{\small
%\centering
\begin{tabular}{c|c c c | c}
& \multicolumn{3}{c}{\textbf{Europarl}} & \multicolumn{1}{|c}{\textbf{Subtitles}}\\
\cline{2-5}
& \textbf{En-Fr} & \textbf{En-Et} & \textbf{En-De} & \textbf{En-Ru} \\
\hline
\hline
\# Sentences & 36.24 & 40.65 &  31.50 & 13.60 \\
%\# En Sentences & 19.99\scriptsize{$\pm$0.49} & 29.72\scriptsize{$\pm$0.74} & &\\
\# Turns & 4.77 & 4.85 & 4.79 & 7.12 \\
%\# En Turns & 2.71\scriptsize{$\pm$0.05} & 3.44\scriptsize{$\pm$0.05} & &\\
Turn Length & 7.12 & 7.92 & 6.16 & 1.68 \\
%Turn Length (whole corpus) & 7.59 & 6.58 & 8.38\\
\hline
\end{tabular}
}
%\vspace{3mm}
\caption{Mean statistics per conversation for training set.}
\label{tab:meanstats}
\end{minipage}
\end{table*}

